Consistency of Proof-of-Stake Blockchains with Concurrent Honest Slot Leaders

We improve the fundamental security threshold of eventual consensus Proof-of-Stake (PoS) blockchain protocols under the longest-chain rule by showing, for the first time, the positive effect of rounds with concurrent honest leaders. Current security analyses reduce consistency to the dynamics of an abstract, round-based block creation process that is determined by three events associated with a round: (i) event $A$: at least one adversarial leader, (ii) event $S$: a single honest leader, and (iii) event $M$: multiple, but honest, leaders. We present an asymptotically optimal consistency analysis assuming that an honest round is more likely than an adversarial round (i.e., $\Pr[S] + \Pr[M] > \Pr[A]$); this threshold is optimal. This is a first in the literature and can be applied to both the simple synchronous communication as well as communication with bounded delays. In all existing consistency analyses, event $M$ is either penalized or treated neutrally. Specifically, the consistency analyses in Ouroboros Praos (Eurocrypt 2018) and Genesis (CCS 2018) assume that $\Pr[S] - \Pr[M] > \Pr[A]$; the analyses in Sleepy Consensus (Asiacrypt 2017) and Snow White (Fin. Crypto 2019) assume that $\Pr[S] > \Pr[A]$. Moreover, all existing analyses completely break down when $\Pr[S] < \Pr[A]$. These thresholds determine the critical trade-off between the honest majority, network delays, and consistency error. Our new results can be directly applied to improve the security guarantees of the existing protocols. We also provide an efficient algorithm to explicitly calculate these error probabilities in the synchronous setting. Furthermore, we complement these results by analyzing the setting where $S$ is rare, even allowing $\Pr[S] = 0$, under the added assumption that honest players adopt a consistent chain selection rule.

==> fork-margin-catalan.tex <==


In this section, we present the connections between Catalan slots and these elements (namely, the ``relative margin''). 
The exposition culminates in Corollary~\ref{coro:catalan-margin-critical} 
which characterizes a Catalan slot in terms of relative margin. 
This directly connects the consistency analysis in Sleepy~\cite{Sleepy} 
and~\cite{LinearConsistency} through the observations made in this paper.



% \input{reach-and-margin}



% We can define the ``forkability'' of a
% characteristic string in terms of its margin.
% Although this definition is not necessary for our presentation, it
% reflects the terminology of existing literature.

% \begin{definition}[Forkable strings]\label{def:forkable}
%   A charactersitic string $w$ is \emph{forkable} if its margin is non-negative, i.e., $\mu(w) \geq 0$.
%   Equivalently, $w$ is forkable if there is a balanced fork for $w$.
% \end{definition}

\subsection{Catalan slots and relative margin}

  Below, we lay down the connection between Catalan slots 
  and relative margin. 
  

